Retrieve, Generate, Evaluate: A Case Study for Medical Paraphrases Generation with Small Language Models

Recent surge in the accessibility of large language models (LLMs) to the general population can lead to untrackable use of such models for medical-related recommendations. Language generation via LLMs models has two key problems: firstly, they are prone to hallucination and therefore, for any medical purpose they require scientific and factual grounding; secondly, LLMs pose tremendous challenge to computational resources due to their gigantic model size. In this work, we introduce pRAGe, a pipeline for Retrieval Augmented Generation and evaluation of medical paraphrases generation using Small Language Models (SLM). We study the effectiveness of SLMs and the impact of external knowledge base for medical paraphrase generation in French.

==> Figures/heatmap-old.tex <==
\begin{figure*}[!ht]
    \centering
    % First row
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_plot.pdf}
        \caption{Caption 1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_plot.pdf}
        \caption{Caption 2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_plot.pdf}
        \caption{Caption 3}
    \end{subfigure}
    
    \vspace{1em} % Space between rows
    
    % Second row
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_plot.pdf}
        \caption{Caption 4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_plot.pdf}
        \caption{Caption 5}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/demo_plot.pdf}
        \caption{Caption 6}
    \end{subfigure}

    \caption{A 2x3 grid of images}
\end{figure*}


==> Tables/Ragcombs.tex <==
\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|ccc}
        \hline
        \textbf{RAG Model} &\textbf{Encoder EN} &\textbf{Decoder EN} & \textbf{Status} \\
        \hline
         \textbf{rag-tok/rag-seq} & \texttt{dpr-ctx}&\texttt{BART} & \\
         \textbf{rag-tok/rag-seq*} & \texttt{dpr-ctx}&\texttt{BioMistral-7B-GGUF}\\
         \textbf{rag-tok/rag-seq*} & \texttt{dpr-ctx}&\texttt{BioMistral-7B}\\
         \textbf{our-rag} & \texttt{all-MiniLM-L6-v2}&\texttt{flan-T5}\\
         \textbf{our-rag*} & \texttt{PubMedBERT}&\texttt{flan-T5}\\
         \textbf{our-rag*} & \texttt{all-MiniLM-L6-v2}&\texttt{BioMistral-7B-GGUF} & $\text{\rlap{$\checkmark$}}\square$\\
         \textbf{our-rag*} & \texttt{all-MiniLM-L6-v2}&\texttt{BioMistral-7B}& $\text{\rlap{$?$}}\square$\\
         \textbf{our-rag} & \texttt{PubMedBERT}&\texttt{BioMistral-7B-GGUF} & $\text{\rlap{$\checkmark$}}\square$\\
         \textbf{our-rag*} & \texttt{PubMedBERT}&\texttt{BioMistral-7B}\\
        \textbf{our-rag*} & \texttt{PubMedBERT}&\texttt{Meditron-7B-GGUF}\\
         \hline
         &\textbf{Encoder FR} &\textbf{Decoder FR}\\
        \hline
         \textbf{rag-tok/rag-seq} & \texttt{sent-CamemBERT}&\texttt{BARThez}\\
         \textbf{rag-tok/rag-seq} & \texttt{Medical-MT5?}&\texttt{BARThez}\\
         \textbf{rag-tok/rag-seq*} & \texttt{DrBERT?}&\texttt{BARThez}\\
         \textbf{our-rag*} & \texttt{sent-CamemBERT}&\texttt{BARThez}\\
         \textbf{our-rag*} & \texttt{Medical-MT5?}&\texttt{BARThez}\\
         \textbf{our-rag*} & \texttt{DrBERT?}&\texttt{BARThez}\\
         \textbf{our-rag*} & \texttt{Medical-MT5?}&\texttt{BioMistral-7B-GGUF}\\
         \textbf{our-rag*} & \texttt{DrBERT?}&\texttt{BioMistral-7B}\\
        \hline
    \end{tabular}}
    \caption{RAG encoder/decoder architectures for the English and French datasets. *= model not yet tested}
\end{table}

==> Tables/prompts.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|cc}
        \hline
        PromptID &  Prompt\\
        \hline
        \st{p2} & \st{Vours êtes un expert en médecine.Expliquez-moi, en termes simples ou paraphrase ou définition :}\\
        p3 & Expliquez-moi, en termes simples ou paraphrase ou définition :\\
        p4 & Expliquez-moi le terme médical en mots simples, par une paraphrase ou une courte définition : \\
        \hline
    \end{tabular}}
    \caption{Prompt setups}
    \label{tab:my_label}
\end{table*}

==> Tables/reports-ft.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{p{3.5cm}|ccc c ccccccccccc}
    \toprule
        Setup & TOKEN& PromptID &  \#status &&-bleu&-bert&-bleurt&-rouge1&-rouge2&-rougL&-rougeLsum&-bleu-p1&-bleu-p2&-bleu-p3&-bleu-p4\\
        \midrule
        \rowcolor{gray!25}
        & \multicolumn{15}{c}{fine-tuned-BIOM-SLERP}\\
        %\small{ fine-tuned-BIOM-SLERP} &25 & p2 & val &   &0.0&0.6928&0.1371&0.1844&0.0696&0.1844&0.1564&0.0937&0.0227&0.0071&0.0009 \\
        \small{ fine-tuned-BIOM-SLERP} &25  & p3 & val &    &\\ 
        \small{ fine-tuned-BIOM-SLERP} &25 & p4 & val &  \\
        %\hdashline
        %\small{ fine-tuned-BIOM-SLERP} &50 & p2 & val &    &0.0016&0.6792&0.1239&0.1768&0.057&0.1768&0.1434&0.0712&0.0158&0.006&0.0025\\
        \small{ fine-tuned-BIOM-SLERP} &50 & p3 & val &    &\\ 
        
        
        \small{ fine-tuned-BIOM-SLERP} &50 & p4 & val &   \\
         %\midrule
         %\small{ fine-tuned-BIOM-SLERP} &25 & p2 & test &   &0.0028&0.6967&0.1417&0.2065&0.0831&0.2065&0.1807&0.1206&0.0358&0.0162&0.0071 \\
        \small{ fine-tuned-BIOM-SLERP} &25 & p3 & test &    \\ 
        \small{ fine-tuned-BIOM-SLERP} &25 & p4 & test &    \\
        %\hdashline
        % \small{ fine-tuned-BIOM-SLERP} &50 & p2 & test &    &0.0031&0.6853&0.1385&0.1836&0.0639&0.1836&0.1508&0.0848&0.0227&0.0099&0.0046\\
        \small{ fine-tuned-BIOM-SLERP} &50 & p3 & test &    \\ 
        \small{ fine-tuned-BIOM-SLERP} &50 & p4 & test &   & \\
        \rowcolor{gray!25}
        & \multicolumn{15}{c}{fine-tuned-orangesum-BARTHEZ}\\
        \midrule
        %fine-tuned-BARTHEZ & 25 & p2 & val & 1063\\
        fine-tuned-BARTHEZ & 25 & p3 & val \\
        fine-tuned-BARTHEZ & 25 & p4 & val \\
        fine-tuned-BARTHEZ & 50 & p3 & val \\
        fine-tuned-BARTHEZ & 50 & p4 & val \\

        fine-tuned-BARTHEZ & 25 & p3 & test \\
        fine-tuned-BARTHEZ & 25 & p4 & test \\
        fine-tuned-BARTHEZ & 50 & p3 & test \\
        fine-tuned-BARTHEZ & 50 & p4 & test \\
        %fine-tuned-BARTHEZ & 50 & p2 & val & 1063\\
        \rowcolor{gray!25}
        & \multicolumn{15}{c}{fine-tuned-BIOM-SLERP-pRAGe}\\
        E:camem D:biomistral & 25& p3 & val  &\\
        E:camem D:biomistral & 50& p3 & val & \\
        E:camem D:biomistral & 25& p4 & val & \\
        E:camem D:biomistral & 50& p4 & val & \\
        E:camem D:biomistral & 25& p3 & test & \\
        E:camem D:biomistral & 50& p3 & test & \\
        E:camem D:biomistral & 25& p4 & test & \\
        E:camem D:biomistral & 50& p4 & test & \\
        \hdashline
        E:drbert D:biomistral & 25& p3 & val \\
        E:drbert D:biomistral & 50& p3 & val & \\
        E:drbert D:biomistral & 25& p4 & val & \\
        E:drbert D:biomistral & 50& p4 & val & \\
        E:drbert D:biomistral & 25& p3 & test & \\
        E:drbert D:biomistral & 50& p3 & test & \\
        E:drbert D:biomistral & 25& p4 & test & \\
        E:drbert D:biomistral & 50& p4 & test & \\
         \rowcolor{gray!25}
        & \multicolumn{15}{c}{fine-tuned-orangesum-BARTHEZ-pRAGe}\\
        E:camem D:barthez & 25& p3 & val &  & \\
        E:camem D:barthez & 50& p3 & val & \\
        E:camem D:barthez & 25& p4 & val & \\
        E:camem D:barthez & 50& p4 & val & \\
        E:camem D:barthez & 25& p3 & test & \\
        E:camem D:barthez & 50& p3 & test & \\
        E:camem D:barthez & 25& p4 & test & \\
        E:camem D:barthez & 50& p4 & test & \\
         \hdashline
        E:drbert D:barthez & 25& p3 & val & \\
        E:drbert D:barthez & 50& p3 & val & \\
        E:drbert D:barthez & 25& p4 & val & \\
        E:drbert D:barthez & 50& p4 & val & \\
        E:drbert D:barthez & 25& p3 & test & \\
        E:drbert D:barthez & 50& p3 & test & \\
        E:drbert D:barthez & 25& p4 & test & \\
        E:drbert D:barthez & 50& p4 & test & \\
         \bottomrule
    \end{tabular}}
    \caption{Evaluation report follows equation \ref{eqn:rag-eval} for each metric (finetuned).}
    \label{tab:eval-reports-ft}
\end{table*}

==> Tables/reports-uft.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{p{3.7cm}|ccc c cccccccccccc}
    \toprule
        Setup & TOKEN& PromptID & Split  &&-bleu&-bert&-bleurt&-rouge1&-rouge2&-rougL&-rougeLsum&-bleu-p1&-bleu-p2&-bleu-p3&-bleu-p4\\
        \midrule
        \rowcolor{gray!25}
        & \multicolumn{15}{c}{no-fine-tuned  -BIOM-SLERP}\\
        %\small{no-fine-tuned  -BIOM-SLERP} &25 & p2 & val   &&0.0&0.6928&0.1371&0.1844&0.0696&0.1844&0.1564&0.0937&0.0227&0.0071&0.0009 \\
        %\small{no-fine-tuned  -BIOM-SLERP} &25  & p3 & val   & &0.0&0.6951&0.1369&0.1887&0.0732&0.1887&0.1593&0.0939&0.022&0.007&0.0006\\ 
        \small{no-fine-tuned  -BIOM-SLERP} &25 & p4 & val   & &0.0&0.6917&0.1411&0.1854&0.0655&0.1854&0.1587&0.0905&0.0214&0.0068&0.0014\\
        %\hdashline
        %\small{no-fine-tuned  -BIOM-SLERP} &50 & p2 & val   & &0.0016&0.6792&0.1239&0.1768&0.057&0.1768&0.1434&0.0712&0.0158&0.006&0.0025\\
        %\small{no-fine-tuned  -BIOM-SLERP} &50 & p3 & val   & &\\ 
        
        
        \small{no-fine-tuned  -BIOM-SLERP} &50 & p4 & val   &&0.0&0.6806&0.1564&0.1744&0.0558&0.1744&0.1403&0.0677&0.0124&0.0033&0.0007\\
         %\midrule
         %\small{no-fine-tuned  -BIOM-SLERP} &25 & p2 & test &    &&0.0028&0.6967&0.1417&0.2065&0.0831&0.2065&0.1807&0.1206&0.0358&0.0162&0.0071 \\
        %\small{no-fine-tuned  -BIOM-SLERP} &25 & p3 & test   &&0.0&0.6961&0.1416&0.2025&0.0786&0.2025&0.1755&0.1149&0.0325&0.013&0.0032 \\ 
        \small{no-fine-tuned  -BIOM-SLERP} &25 & p4 & test &   &0.0028&0.6936&0.1423&0.1955&0.0702&0.1955&0.1689&0.1127&0.0311&0.014&0.0073\\
        %\hdashline
        % \small{no-fine-tuned  -BIOM-SLERP} &50 & p2 & test &    & &0.0031&0.6853&0.1385&0.1836&0.0639&0.1836&0.1508&0.0848&0.0227&0.0099&0.0046\\
        %\small{no-fine-tuned  -BIOM-SLERP} &50 & p3 & test &    &0.0075&0.6846&0.1352&0.1848&0.0668&0.1848&0.153&0.0896&0.0277&0.0151&0.0102\\ 
        \small{no-fine-tuned  -BIOM-SLERP} &50 & p4 & test &   & 0.003&0.6804&0.1521&0.1793&0.0597&0.1793&0.145&0.0803&0.0205&0.0084&0.0042\\
        \rowcolor{gray!25}
        & \multicolumn{15}{c}{no-fine-tuned  -BARTHEZ}\\
        \midrule
        %no-fine-tuned  -BARTHEZ & 25 & p2 & val  \\
        %\small{no-fine-tuned  -BARTHEZ} & 25 & p3 & val  &&0.0&0.6316&0.0851&0.1137&0.0178&0.1137&0.0936&0.0591&0.004&0.0013&0.0003\\
        %\small{no-fine-tuned  -BARTHEZ} & 50 & p3 & val &&0.0&0.6316&0.0851&0.1137&0.0178&0.1137&0.0936&0.0591&0.004&0.0013&0.0003 \\
        \small{no-fine-tuned  -BARTHEZ} & 25 & p4 & val  &&0.0&0.643&0.1213&0.084&0.0189&0.084&0.0784&0.0361&0.0029&0.0012&0.0002\\
        \small{no-fine-tuned  -BARTHEZ} & 50 & p4 & val  &&0.0&0.643&0.1213&0.084&0.0189&0.084&0.0784&0.0361&0.0029&0.0012&0.0002\\
        %\small{no-fine-tuned  -BARTHEZ} & 25 & p3 & test &&0.0&0.6244&0.0783&0.0946&0.0118&0.0946&0.0815&0.0514&0.0035&0.0007&0.0002 \\
        %\small{no-fine-tuned  -BARTHEZ} & 50 & p3 & test &&0.0&0.6244&0.0783&0.0946&0.0118&0.0946&0.0815&0.0514&0.0035&0.0007&0.0002 \\
        \small{no-fine-tuned  -BARTHEZ} & 25 & p4 & test &&0.0&0.634&0.0996&0.0699&0.0071&0.0699&0.0635&0.0351&0.0018&0.0002&0.0 \\
        \small{no-fine-tuned  -BARTHEZ} & 50 & p4 & test  &&0.0&0.634&0.0996&0.0699&0.0071&0.0699&0.0635&0.0351&0.0018&0.0002&0.0\\
        %no-fine-tuned  -BARTHEZ & 50 & p2 & val  \\
        \rowcolor{gray!25}
        & \multicolumn{15}{c}{no-fine-tuned  -BIOM-SLERP-pRAGe}\\
        %E:camem D:biomistral & 25& p3 & val    &&0.0&0.6852&0.1363&0.139&0.0479&0.139&0.1209&0.0728&0.0168&0.0052&0.0003\\
        %E:camem D:biomistral & 50& p3 & val   &&0.0001&0.6718&0.1537&0.13&0.0354&0.13&0.1032&0.0604&0.0119&0.0033&0.0005\\
        E:camem D:biomistral & 25& p4 & val &&0.0&0.6859&0.1332&0.1418&0.047&0.1418&0.1232&0.0737&0.0165&0.0057&0.0003  \\
        E:camem D:biomistral & 50& p4 & val   &&0.0003&0.6746&0.1629&0.1357&0.0366&0.1357&0.1096&0.0621&0.0107&0.0032&0.0006\\
        %E:camem D:biomistral & 25& p3 & test & &0.0004&0.6914&0.1499&0.1785&0.0712&0.1785&0.1567&0.0922&0.0254&0.0093&0.0017  \\
        %E:camem D:biomistral & 50& p3 & test &&0.0001&0.6797&0.1495&0.1588&0.0562&0.1588&0.1315&0.0694&0.016&0.006&0.0017  \\
        E:camem D:biomistral & 25& p4 & test  &&0.0&0.6909&0.1472&0.1741&0.0592&0.1741&0.1494&0.0948&0.0232&0.0094&0.0018 \\
        E:camem D:biomistral & 50& p4 & test &&0.0001&0.6817&0.1587&0.1621&0.0488&0.1621&0.1306&0.0736&0.0156&0.0054&0.0012  \\
        \hdashline
        %E:drbert D:biomistral & 25& p3 & val    &&0.0&0.678&0.1457&0.1052&0.0342&0.1052&0.0914&0.0567&0.0117&0.0032&0.0\\
        %E:drbert D:biomistral & 50& p3 & val &&0.0&0.6649&0.1536&0.0958&0.0257&0.0958&0.0779&0.0474&0.0086&0.0026&0.0004  \\
        E:drbert D:biomistral & 25& p4 & val &&0.0&0.6738&0.138&0.0952&0.0269&0.0952&0.083&0.0501&0.011&0.003&0.0001  \\
        E:drbert D:biomistral & 50& p4 & val  &&0.0&0.6616&0.1482&0.0899&0.0211&0.0899&0.0712&0.0415&0.0069&0.0019&0.0003 \\
        %E:drbert D:biomistral & 25& p3 & test  &&0.0005&0.6809&0.145&0.1088&0.0374&0.1088&0.0954&0.0626&0.0138&0.0043&0.0014 \\
        %E:drbert D:biomistral & 50& p3 & test &&0.0012&0.669&0.1459&0.1&0.0281&0.1&0.0793&0.049&0.0106&0.0039&0.0021  \\
        E:drbert D:biomistral & 25& p4 & test &&0.0&0.6744&0.1308&0.1086&0.0352&0.1086&0.0913&0.0574&0.0115&0.0037&0.0007  \\
        E:drbert D:biomistral & 50& p4 & test &&0.0&0.6646&0.1363&0.1008&0.029&0.1008&0.0796&0.0465&0.0091&0.0033&0.0014  \\
         \rowcolor{gray!25}
        & \multicolumn{15}{c}{no-fine-tuned  orangesum-BARTHEZ-pRAGe}\\
        %E:camem D:barthez & 25& p3 & val    & &0.0&0.6667&0.1042&0.1411&0.0277&0.1411&0.1143&0.0588&0.0051&0.0008&0.0001\\
        %E:camem D:barthez & 50& p3 & val  &&0.0&0.666&0.1433&0.1409&0.0279&0.1409&0.1124&0.0565&0.0051&0.0009&0.0001 \\
        E:camem D:barthez & 25& p4 & val  &&0.0&0.6565&0.0775&0.1385&0.0269&0.1385&0.1106&0.0575&0.0063&0.0022&0.0001 \\
        E:camem D:barthez & 50& p4 & val  &&0.0&0.6593&0.1472&0.1457&0.0391&0.1457&0.1171&0.0568&0.007&0.0022&0.0002 \\
        %E:camem D:barthez & 25& p3 & test  &&0.0&0.6647&0.0884&0.1319&0.0226&0.1319&0.1084&0.0685&0.0085&0.002&0.0004 \\
        %E:camem D:barthez & 50& p3 & test   &&0.0&0.6625&0.1266&0.1307&0.0227&0.1307&0.1064&0.0638&0.0069&0.0013&0.0002\\
        E:camem D:barthez & 25& p4 & test  &&0.0&0.6521&0.0734&0.1187&0.0188&0.1187&0.0987&0.0538&0.0045&0.0011&0.0002 \\
        E:camem D:barthez & 50& p4 & test &&0.0&0.6525&0.1127&0.1164&0.0179&0.1164&0.0955&0.049&0.0038&0.0011&0.0002  \\
         \hdashline
        %E:drbert D:barthez & 25& p3 & val &&0.0&0.6478&0.0446&0.1125&0.0217&0.1125&0.099&0.0523&0.0059&0.002&0.0014  \\
        %E:drbert D:barthez & 50& p3 & val  &&0.0&0.6447&0.0558&0.1133&0.0195&0.1133&0.0973&0.0485&0.0057&0.002&0.0014 \\
        E:drbert D:barthez & 25& p4 & val &&0.0&0.6397&0.0258&0.1209&0.0109&0.1209&0.0958&0.0459&0.0033&0.0001&0.0  \\
        E:drbert D:barthez & 50& p4 & val  &&0.0&0.6329&0.0636&0.1124&0.0109&0.1124&0.0889&0.0402&0.0024&0.0002&0.0 \\
        %E:drbert D:barthez & 25& p3 & test &&0.0&0.6583&0.0414&0.0984&0.0067&0.0984&0.0813&0.0457&0.0015&0.0001&0.0  \\
        %E:drbert D:barthez & 50& p3 & test  &&0.0&0.6583&0.0682&0.0986&0.007&0.0986&0.0819&0.0445&0.0017&0.0001&0.0 \\
        E:drbert D:barthez & 25& p4 & test &&0.0&0.6414&0.0235&0.1027&0.0047&0.1027&0.0811&0.0446&0.0005&0.0&0.0  \\
        E:drbert D:barthez & 50& p4 & test  &&0.0&0.6517&0.0501&0.1096&0.0074&0.1096&0.0864&0.048&0.0016&0.0&0.0 \\
        %\midrule
        %\\
         \bottomrule
    \end{tabular}}
    \caption{Evaluation report follows equation \ref{eqn:rag-eval} for each metric (without fine tuning).}
    \label{tab:eval-reports-uft}
\end{table*}
